Athermal package for OH suppression filters in astronomy part 1: design

We present the design of an athermal package for fiber Bragg grating (FBG)filters fabricated at our Institute for use in ground-based near-infrared (NIR) telescopes. Aperiodic multichannel FBG filters combined with photonic lanterns can effectively filter out extremely bright atmospheric hydroxyl (OH) emission lines that severely hinder ground-based NIR observations. While FBGs have the capability of filtering specific wavelengths with high precision, due to their sensitivity to temperature variations, the success in their performance as OH suppression filters depends on a suitable athermal package that can maintain the deviations of the FBG wavelengths from that of the OH emission lines within sub-picometer accuracy over a temperature range of about 40 K. (i.e. 263 K to 303 K). We aim to develop an athermal package over the aforementioned temperature range for an optical fiber consisting of multichannel FBGs for a maximum filter length of 110 mm. In this work, we demonstrate the complete design methodology of such a package. First, we developed a custom-built test rig to study a wide range of critical physical properties of the fiber, such as strain and temperature sensitivities, elastic modulus, optimum fiber pre-tension, and adhesion performance.Next, we used these data to confirm the athermal response of an FBG bonded on the test rig from room temperature to 313 K. Based on this study, we developed a computer-aided design (CAD) model of the package and analyzed its athermal characteristics with a suitable selection of materials and their nominal dimensions using finite element analysis (FEA). We finally discuss the novel aspects of the design to achieve high-precision thermal stabilization of these filters in the temperature range of interest.

==> Content/Methode.tex <==

%\section{Method}
%\label{Method}

\subsubsection{Test the glue stability}

For the experimental phase, the same FBG fiber had to be used each time for the different experiments, the FBG had to be mounted and dismounted more often due to the repetitiveness and accuracy of the experiments. In addition, the experimental phase required a large number of FBGs, which requires a lot of effort for the manufacture process.

The challenge was to find a holding method that would allow the same FBG to be mounted and secured to the various test stands without damaging the optical fiber and the FBG.
After testing various commercially available Holders(should i write hier the thorlabs??), such as magnetic or friction holders, it was found that the glass Fiber  slipped at the required preload or the glas Fiber was damaged.

Another method of attaching the glass mount that has worked is with glue,the glue used, Pattex sekunden kleber from the company Henkel, has passed all the tests described below.To disolving the glue will be used acetone.See Figure %%\ref{glue\_test}

\begin{figure}[h]
{\centering
%includesvg[width=0.6]{Abbildungen/plot_lichtwellenleiter_messung.eps}
%includesvg[width=0.6]{Abbildungen/plot_lichtwellenleiter_messung.svg}
\includegraphics[width=0.8\textwidth]{pictures/glue_test.png} \label{Glue Test Bensch}
\caption[glue\_test]{Glue Test Bensch}
\end{figure}


The optical fiber was glued to the fiber holder HFF001-M from Thorlabs, which are made of aluminum with an anodized surface, the adhesive length is 3 to 4 mmm.

The adhesion of the optical fibers to the aluminum components was tested with different loads, all loads are higher than the future prestressing that the optical fiber will experience.The entire test stand was set up on a stable optical bench in a temperature-controlled room at 20 °C +- 3 °C.


The Fiber holder HFF001-M were bolted on each side to the M-DS25-XYZ Compact Metric Dovetail Linear Stage, which was bolted on the same side to a common component (Conector Part) to create a stable and consistent mechanical system.

At the beginning of the test, there was mecanical tension in the FBG and light was reflected at a wavelength of xxx.

The two bonding points were poulled xxx mm apart in Z direction using the XYZ stage.
The new pulling force or mecanical tension on the optical fiber caused a shift of the reflected wavelength of xxx Pm to the red.???The stage was fixed with the supplied fixing screws and the fiber glass with the FBG grating was held under this tension for 24 hours.The reflected wavelength were controlled and tracked all the time during the experiment using a Optical complex spectrum analyzer Apex AP 2683A with a measurement accuracy of xxxxxpm

The deviation of the reflected wavelength from the initial wavelength after 24 hours was xxxpm. The minimal deviation from the initial reflected wavelength is due to the temperature change in the room.\\
From the results of the experiment, it can be said that the glue Pattex from the company Henkel provides a good support for the optical fiber and the adhesive surface of 2 mm is enough to hold the necessary preload of the optical mounts without slipping.



\subsubsection{Test bench in a controlled environment for measuring 
The strain and temperature response of the FBG}

One of the uncertainties that we had in calculating the necessary compensation was the expansion or contraction of the optical fiber with respect a change in temperature (\(\Delta T\)), in other words, the coefficient of thermal expansion as well as the thermo-optical coefficient.
One had the values for the coefficient of thermal expansion  $5x10^{-7}/\degree{C}$ and for the thermo-optical coefficient  $7x10^{6}/\degree{C}.$ of xxxxxxx (hier come the source TERAXION)

Unknown was also  the side effects of the UV laser writings of the FBG and the possible changes in the mechanical and physical properties of the optical fiber.We designed, manofactured and mounted a test bench to determine the physical properties of our own optical fiber after our writing porocess, in this case was the main target know the CTE of our optical fiber, to achieve greater accuracy in the FEM analysis and to obtain more accurate  themperarture compensation later in the athermal package.
See picture xxxxxx(hier kommt die foto nur mit dem fiber auf dem hotplate

\begin{figure}[h]
{\centering
%includesvg[width=0.6]{Abbildungen/plot_lichtwellenleiter_messung.eps}
%includesvg[width=0.6]{Abbildungen/plot_lichtwellenleiter_messung.svg}
\includegraphics[width=0.8\textwidth]{pictures/temperature_sensitivity.png} %\label{abb:system}
\caption[temperature\_sensitivity]{Temperature Sensitivity Test Bensch}
\end{figure}




The fiber was heated and cooled using the Temperature-Controlled Breadboard PTC1/M from the company Thorlabs. During the experiments, large intervals were chosen between the temperature steps to achieve better accuracies.With the temperature change, the reflected wavelength has changed, these values could be read in the spectrum analyzer, 
We repeated the experiment 4 ? times, the results are the average of the 4 different values.
see Table xxxxxx

the Overall Temperature Sensitivity of our optical fiber after the FBG writing is  9,795833333 pm/\degree{C}.





\subsubsection {A manual control of the fiber expansion/contraction to compensate for decrease/increase in temperature}_(i think we need hier other subtitle)

The optical fiber was glued at 2 different points on the  fiber holder using Pattex sekunden kleber (super glue better???ß) from the company Henkel, so that the FBG is in the middle of the two glued points.Using the XYZ stage, the two adhesive points were pulled away from each other, in the Z direction, the necessary pretension was  was achieved with the spectral analyzer, and the XY table secured with the screw provided for this purpose.


Using this experimental setup, we also measured an important parameter that will improve the accuracy of athermalization in the future. This is the necessary compensation value, i.e. exactly how much the athermal package should push or pull the optical fibers so that the set reflected waves remain constant after the temperature changes, taking into account the tolerances.
see picture xxxxxxxxxxxxxxxxxx



\begin{figure}[h]
{\centering
%includesvg[width=0.6]{Abbildungen/plot_lichtwellenleiter_messung.eps}
%includesvg[width=0.6]{Abbildungen/plot_lichtwellenleiter_messung.svg}
\includegraphics[width=0.8\textwidth]{pictures/compesation_testbensch.png} %\label{abb:system}
\caption[compensation\_test\_bench]{Compensation Test Bench}
\end{figure}

The Temperature-Controlled Breadboard PTC1/M was set to different temperatures, so the reflected wavelength shifted with the temperature change, the red or green shift was seen and tracked exactly in the xxxxx spectrum analyzerApex AP 2683A. 
When the temperature stabilized, the xyz stage was moved in the x direction until the original wavelength was restored. When the temperature stabilized, the xyz stage was moved in the x direction until the original wavelength was restored. The displacement of the stage in the Z direction was measured with the confocaler sensor. (See the results are in the table xxxxxxx)\\

\subsubsetction{Pre-strain selection}

A Pre-strain in the optical fiber is necessary in case of compensation when the temperature increase, in this moment the athermal package should compensate to hold the selected wavelength reflection constant.The compensation takes place when the athermalpackage compresses the optical fibers

by adding pressure to the glass fibers to bring the distances between the gratings back to the set position. If the glass fibers in the athermal package are not tensioned, the compensation would cause the glass fibers to bend and the distance between the grids to change.

Due to the opto-elastic effect, however, this prestressing is also counterproductive and should be kept as low as possible
ause the glass fibers to bend and the distance between the grids to change.

\subsubsection{CAD design and ANSYS modeling for material dimension selection}
To design the Athermal package, we first performed a state-of-the-art research. During the research, several solutions were found, but none that met our requirements, length of the FBG, repeatability, adjustable preload, and the ability to write the FBG after the optical fiber is clamped and in final position.
Based on these requirements, we created several CAD models that met the requirements and selected the current one.
The model was created using the Inventor computer program and was designed with a view to future FEM calculations.
Once the basic model was ready, calculations were made to determine the exact dimensions of each component.




==> Content/Theory.tex <==
%\section{Theory}
%\label{Theory}
The fiber Bragg grating (FBG) is a periodic microstructure in into a photosensitive optical fiber, this system enables precise wavelength filtering of the light transmitted through the fiber. The light from a source with a large bandwidth is introduced into the optical fiber, only light of a very limited spectral width around the Bragg wavelength is reflected at the grating. The rest of the light continues its path through the optical fiber without attenuation to the next Bragg grating.

A fiber Bragg grating (FBG) is inscribed in different ways – 1) phase mask technique,2) interferometry technique, 3) direct inscription technique. In all these methods, a precise fabrication of an FBG depends on how the fiber is aligned with respect to the interference fringes during the inscription process. The wave length that is reflected is directly dependent on the distance between the gratings.\\

For a uniform grating the Bragg wavelength is represented as, 
$\lambda$_B=2n$\Lambda$\\
Where $\Lambda$ is the spatial period of the index modulation in the fiber grating and \textit{n} is the average effective refractive index of the guided mode at the position of the grating.\\

The distance between the gratings varies depending on the temperature of the optical fiber because the lenhth optical fiber increases or decreases depending on the temperature change.
\subsection{ Thermo-optic Effects}

As mentioned the distance between the gratings varies depending on the temperatuture and thus the reflected wavelength There are two effects known as thermo-optic $\xi$ and thermal expansion $\alpha_{f}$ that shift the Bragg wavelength to longer or shorter wavelength when there is a temperature variation around the FBG.\\

The shift in Bragg wavelength due to temperature which is a result of the above mentioned two combined effects is given as,$\frac{\Delta\lambda_B}{\lambda_B}= $\alpha_f \Delta$T+ \xi\Delta$T\\

Where $\alpha_{f}$ is the coefficient of thermal expansion and $\xi$ is the thermo-optic coefficient.\\
Typical values for a silica fiber are $\alpha_{f} =7x10^{6}/\degree{C}$ and $\xi$ = $5x10^{-7}/\degree{C}$.\\

The net temperature dependence of the Bragg wavelength for a grating written in a typical silica-based fiber is thus about +10 pm/\degree{C}.\\

\subsection{Thermo-optic Effect}
This is another relevant efect, The reflected light wavelength also increases when the fiber is stretched under tensile force which produce a  tension in the optical fiber, leading to an increase in the modulation period Λ. This increase is partially offset by an ensuing reduction in the refractive index n through. the photo-elastic effect is described by the next equation:\\
$\frac{\Delta\lambda_B}{\lambda_B}$= $\Delta\epsilon- $P_e$\Delta\epsilon$\\
Where $p_e$ is the photo-elastic constant and $\Delta\epsilon$=$\frac{\Delta L}{L}$ is the longitudinal strain in the fiber resulting from the applied tensile force, where L is the fiber length. The first term on the right side  of the equation corresponds the change in the modulation period n period due to the fiber elongation, whereas the second one corresponds to the change in the average refractive index due to the photo-elastic effect. A typical value for the photo-elastic constant $p_e$ in a germanosilicate fiber is about 0.22, leading to a Bragg wavelength sensitivity of 1.2 pm/microstrain at 1550 nm.





